FairQueue: Rethinking Prompt Learning for Fair Text-to-Image Generation

Recently, prompt learning has emerged as the state-of-the-art (SOTA) for fair text-to-image (T2I) generation. Specifically, this approach leverages readily available reference images to learn inclusive prompts for each target Sensitive Attribute (tSA), allowing for fair image generation. In this work, we first reveal that this prompt learning-based approach results in degraded sample quality. Our analysis shows that the approach's training objective -- which aims to align the embedding differences of learned prompts and reference images -- could be sub-optimal, resulting in distortion of the learned prompts and degraded generated images. To further substantiate this claim, as our major contribution, we deep dive into the denoising subnetwork of the T2I model to track down the effect of these learned prompts by analyzing the cross-attention maps. In our analysis, we propose a novel prompt switching analysis: I2H and H2I. Furthermore, we propose new quantitative characterization of cross-attention maps. Our analysis reveals abnormalities in the early denoising steps, perpetuating improper global structure that results in degradation in the generated samples. Building on insights from our analysis, we propose two ideas: (i) Prompt Queuing and (ii) Attention Amplification to address the quality issue. Extensive experimental results on a wide range of tSAs show that our proposed method outperforms SOTA approach's image generation quality, while achieving competitive fairness. More resources at FairQueue Project site: https://sutd-visual-computing-group.github.io/FairQueue

==> Section/Backup_Content.tex <==
\begin{table*}[!t]
    \centering
    \caption{{\bf Evaluating \ours against \itigen, Hard-Prompts (HP) and Stable Diffusion Base Prompt (BP).} We utilize {\it FD:} Fairness Discrepancy ($\downarrow$), {\it TA:} Text-Alignment ($\uparrow$) and {\it DS:} DreamSim ($\downarrow$) to determine the fairness, quality, and semantic preservation, respectively.
    For FD a combination of CLIP \cite{radford2021clip}, off-the-shelf classifier \cite{FengTRUSTFAIR,karkkainen2021fairface} and human evaluator were utilized as tSA classifier.
    For TA we utilize CLIP \cite{radford2021clip} as the feature extractor.
    %For FD and TA a CLIP-Image Encoder is utilized as a feature extractor. 
    Overall, our proposed method demonstrates the best ability to balance between sample quality and fairness, while preserving the semantics of the original base-prompt $T$. {\bf Bold} and  \underline{underline} values indicate the first and second best results.
    }
    \resizebox{\textwidth}{!}{
    \begin{tabular}{cc cccc }
    \toprule
    \multicolumn{6}{c}{{\bf Single-Target Binary tSA}}\\
    \midrule
    & & BP & HP & \itigen & Ours    \\
    \midrule
    % Gender %
    \multirow{4}{*}{{\bf Gender}}
    & \multicolumn{1}{r|}{FD  ($\downarrow$)} & $0.130 \pm 0.012$  & $\mathbf{1.41 \text{e}^{-3} \pm 6.1 \text{e}^{-3}}$ & $\mathbf{1.41 \text{e}^{-3} \pm 4.2 \text{e}^{-3}}$ & $\mathbf{1.41 \text{e}^{-3} \pm 3.8 \text{e}^{-3}}$ \\
    & \multicolumn{1}{r|}{TA  ($\uparrow$)} & $\mathbf{0.712 \pm 1.1\text{e}^{-2}}$ & \underline{$0.699 \pm x.xx$} & $0.655 \pm x.xx$ & $0.676 \pm x.xx$ \\
    & \multicolumn{1}{r|}{FID ($\downarrow$)} & $97.04 \pm 2.32$ & $89.0 \pm x.xx$ & \underline{${78.9 \pm x.xx}$} & ${\bf 78.3 \pm x.xx}$ \\
    & \multicolumn{1}{r|}{DS ($\downarrow$)} & - & \underline{$0.318 \pm x.xx$} & $0.337 \pm x.xx$ & $\mathbf{0.308 \pm x.xx}$ \\
    \midrule 
    % Young %
    \multirow{4}{*}{{\bf Young}}
    & \multicolumn{1}{r|}{FD ($\downarrow$)} & $0.681 \pm 2.1\text{e}^{-2}$ & $\mathbf{2.81 \text{e}^{-3} \pm 1.4 \text{e}^{-3}}$ & \underline{$1.31 \text{e}^{-2} \pm 8.1\text{e}^{-3}$} & $1.55 \text{e}^{-2} \pm 3.8\text{e}^{-3}$  \\
    & \multicolumn{1}{r|}{TA ($\uparrow$)}   & $\mathbf{0.712 \pm 1.1\text{e}^{-2}}$ & $0.672 \pm x.xx$ & $0.653 \pm x.xx$ & \underline{$0.678 \pm x.xx$}  \\
    & \multicolumn{1}{r|}{FID ($\downarrow$)} & $97.04 \pm 2.32$ & $83.58 \pm x.xx$ & \underline{$82.88 \pm x.xx$} & ${\bf 75.28 \pm x.xx}$\\
    & \multicolumn{1}{r|}{DS ($\downarrow$)} & - & \underline{$0.392 \pm x.xx$} & $0.552 \pm x.xx$ & $\mathbf{0.370 \pm x.xx}$\\
     % Smiling %
    \midrule
    \multirow{4}{*}{{\bf Smiling}}
    & \multicolumn{1}{r|}{FD ($\downarrow$)} & $0.410 \pm 1.1 \text{e}^{-2}$ & $\mathbf{8.4\text{e}^{-3} \pm 1.0 \text{e}^{-3}}$  & $0.124 \pm 9.2 \text{e}^{-3}$ & \underline{$6.9 \text{e}^{-2} \pm 4.2 \text{e}^{-3}$}\\
    & \multicolumn{1}{r|}{TA ($\uparrow$)}   & $\mathbf{0.712 \pm 1.1\text{e}^{-2}}$ & $0.672 \pm x.xx$ & $0.605 \pm x.xx$ & $\mathbf{0.674 \pm x.xx}$\\
    & \multicolumn{1}{r|}{FID ($\downarrow$)} & $97.04 \pm 2.32$  & ${\bf 79.82 \pm x.xx}$ & $88.63 \pm x.xx$ & \underline{$80.01 \pm x.xx$}\\
    & \multicolumn{1}{r|}{DS ($\downarrow$)} &  - & \underline{$0.323 \pm x.xx$}    & $0.557 \pm x.xx$ & $\mathbf{0.284 \pm x.xx}$\\
    % Pale Skin %
    \midrule
    \multirow{4}{*}{{\bf High Cheekbones}}
    & \multicolumn{1}{r|}{FD ($\downarrow$)}  & $0.557 \pm 3.2\text{e}^{-2}$ & ${\bf 3.68 \text{e}^{-3} \pm x.xx}$ &  $0.318 \pm x.xx$ & \underline{$4.92 \text{e}^{-3} \pm x.xx$}\\
    & \multicolumn{1}{r|}{TA ($\uparrow$)}    & $\mathbf{0.712 \pm 1.1\text{e}^{-2}}$ & $0.672 \pm x.xx$ & $0.595 \pm x.xx$ & \underline{$0.685 \pm x.xx$}\\
    & \multicolumn{1}{r|}{FID ($\downarrow$)} & $97.04 \pm 2.32$  & $80.32 \pm x.xx$ & \underline{$86.42 \pm x.xx$} & ${\bf 79.73 \pm x.xx}$\\
    & \multicolumn{1}{r|}{DS ($\downarrow$)}  & - & \underline{$0.332 \pm x.xx$} & $0.538 \pm x.xx$ & ${\bf 0.330 \pm x.xx}$\\ 
    \midrule
    \multirow{4}{*}{{\bf Pale Skin}}
    & \multicolumn{1}{r|}{FD ($\downarrow$)} & $0.568 \pm 2.4 \text{e}^{-2}$ & $0.591 \pm 4.3 \text{e}^{-2}$ & $\mathbf{1.41 \text{e}^{-3} \pm 1.2 \text{e}^{-3}}$ & $\mathbf{1.41 \text{e}^{-3} \pm 1.0 \text{e}^{-3}}$ \\
    & \multicolumn{1}{r|}{TA ($\uparrow$)}   & $\mathbf{0.712 \pm 1.1\text{e}^{-2}}$ & $0.660 \pm x.xx$ & $0.646 \pm x.xx$ & \underline{$0.666 \pm x.xx$}\\
    & \multicolumn{1}{r|}{FID ($\downarrow$)} & \underline{$97.04 \pm 2.32$} & $105.42 \pm x.xx$ & $101.29 \pm x.xx$ & ${\bf 97.03 \pm x.xx}$ \\
    & \multicolumn{1}{r|}{DS ($\downarrow$)} & - & $\mathbf{0.387 \pm x.xx}$ & $0.525 \pm x.xx$ & \underline{$0.408 \pm x.xx$}\\
    % Eyeglasses %
    \midrule
    \multirow{4}{*}{{\bf Eyeglasses}}
    & \multicolumn{1}{r|}{FD ($\downarrow$)} & $0.554 \pm x.xx$ & $0.683 \pm x.xx$ & $\mathbf{1.41 \text{e}^{-2} \pm x.xx}$ & \underline{$2.54 \text{e}^{-2} \pm x.xx$} \\
    & \multicolumn{1}{r|}{TA ($\uparrow$)}   & $\mathbf{0.712 \pm 1.1\text{e}^{-2}}$ & $0.669 \pm x.xx$ & $0.654 \pm x.xx$ & \underline{$0.670 \pm x.xx$}\\
    & \multicolumn{1}{r|}{FID ($\downarrow$)} & $97.04 \pm 2.32$  & $89.78 \pm x.xx$ & \underline{$83.53 \pm x.xx$} & ${\bf 79.40 \pm x.xx}$\\
    & \multicolumn{1}{r|}{DS ($\downarrow$)} & - & \underline{$0.467 \pm x.xx$} & $0.486 \pm x.xx$ & $\mathbf{0.391 \pm x.xx}$\\
    % Mustache %
    \midrule
    \multirow{4}{*}{{\bf Mustache}}
    & \multicolumn{1}{r|}{FD ($\downarrow$)}  & $0.639 \pm 4.2\text{e}^{-2}$\\
    & \multicolumn{1}{r|}{TA ($\uparrow$)}    & $\mathbf{0.712 \pm 1.1\text{e}^{-2}}$\\
    & \multicolumn{1}{r|}{FID ($\downarrow$)} & $97.04 \pm 2.32$  \\
    & \multicolumn{1}{r|}{DS ($\downarrow$)}  & -\\ 
    \midrule
    \multicolumn{6}{c}{{\bf Multi-Target Binary tSA}}\\
    \midrule
    \multirow{4}{*}{{\bf Gender x Young}}
    & \multicolumn{1}{r|}{FD ($\downarrow$)} & $0.493 \pm x.xx$ & \underline{$1.46\text{e}^{-2} \pm x.xx$} & $3.91\text{e}^{-2} \pm x.xx$ & ${\bf 1.24\text{e}^{-2} \pm x.xx}$  \\
    & \multicolumn{1}{r|}{TA ($\uparrow$)}   & ${\bf 0.712 \pm 1.1\text{e}^{-2}}$ & $0.683 \pm x.xx$ & $0.668 \pm x.xx$ & \underline{$0.686 \pm x.xx$}    \\
    & \multicolumn{1}{r|}{FID ($\downarrow$)} & $97.04 \pm 2.32$  \\
    & \multicolumn{1}{r|}{DS ($\downarrow$)} & - & \underline{$0.408 \pm x.xx $} & $0.458 \pm x.xx$ & ${\bf 0.373 \pm x.xx}$\\
    \midrule
    \multirow{4}{*}{\bf \shortstack{Gender x Young \\ x Eyeglasses}}
    & \multicolumn{1}{r|}{FD ($\downarrow$)} & $0.566 \pm x.xx$ & $0.289 \pm x.xx$ & \underline{$0.257 \pm x.xx$} & ${\bf 0.208 \pm x.xx}$ \\
    & \multicolumn{1}{r|}{TA ($\uparrow$)}   & ${\bf 0.712 \pm 1.1\text{e}^{-2}}$ & $0.658 \pm x.xx$ & $0.654 \pm x.xx$ & \underline{$0.671 \pm x.xx$}\\
    & \multicolumn{1}{r|}{FID ($\downarrow$)} & $97.04 \pm 2.32$  \\
    & \multicolumn{1}{r|}{DS ($\downarrow$)} & - & $0.490 \pm x.xx$ & \underline{$0.475 \pm x.xx$} & ${\bf 0.360 \pm x.xx}$ \\
    \midrule
    \multirow{4}{*}{\bf \shortstack{Gender x Young x\\ Eyeglasses x Smiling}}
    & \multicolumn{1}{r|}{FD ($\downarrow$)} & $0.476 \pm x.xx$ & $0.204 \pm x.xx$ & \underline{$0.190 \pm x.xx$} & ${\bf 0.168 \pm x.xx}$ \\
    & \multicolumn{1}{r|}{TA ($\uparrow$)}   & ${\bf 0.712 \pm 1.1\text{e}^{-2}}$ & $0.660 \pm x.xx$ & $0.643 \pm x.xx$ & \underline{$0.661 \pm x.xx$} \\
    & \multicolumn{1}{r|}{FID ($\downarrow$)}  & $97.04 \pm 2.32$ \\
    & \multicolumn{1}{r|}{DS ($\downarrow$)} & - & $0.492 \pm x.xx$ & \underline{$0.475 \pm x.xx$} & ${\bf 0.379 \pm x.xx}$\\
    \midrule
    \multicolumn{6}{c}{{\bf Multi-Target Multi-Class tSA}}\\
    \midrule
    \multirow{4}{*}{{\bf Gender x Age}}
    & \multicolumn{1}{r|}{FD ($\downarrow$)} & $0.452 \pm x.xx$ & - & $0.242 \pm x.xx$ & $0.208 \pm x.xx$\\
    & \multicolumn{1}{r|}{TA ($\uparrow$)}   & $0.712 \pm 1.1\text{e}^{-2}$ & - & $0.659 \pm x.xx$ & $0.672 \pm x.xx$ \\
    & \multicolumn{1}{r|}{FID ($\uparrow$)}  & $97.04 \pm 2.32$ & - & $58.24 \pm x.xx$ & $58.81\pm x.xx$  \\
    & \multicolumn{1}{r|}{DS ($\downarrow$)} & - & - & $0.445 \pm x.xx$ & $0.359 \pm x.xx$  \\
    \midrule
    \multirow{4}{*}{{\bf Gender x Skin tone}}
    & \multicolumn{1}{r|}{FD ($\downarrow$)}  \\
    & \multicolumn{1}{r|}{TA ($\uparrow$)}    \\
    & \multicolumn{1}{r|}{FID ($\uparrow$)}    \\
    & \multicolumn{1}{r|}{DS ($\downarrow$)}  \\
    \bottomrule
    \end{tabular}
    }
    \label{tab:ours_vs_ITIGen}
\end{table*}
